Usefulness of the Age-Structured SIR Dynamics in Modelling COVID-19

We examine the age-structured SIR model, a variant of the classical Susceptible-Infected-Recovered (SIR) model of epidemic propagation, in the context of COVID-19. In doing so, we provide a theoretical basis for the model, perform an empirical validation, and discover the limitations of the model in approximating arbitrary epidemics. We first establish the differential equations defining the age-structured SIR model as the mean-field limits of a continuous-time Markov process that models epidemic spreading on a social network involving random, asynchronous interactions. We then show that, as the population size grows, the infection rate for any pair of age groups converges to its mean-field limit if and only if the edge update rate of the network approaches infinity, and we show how the rate of mean-field convergence depends on the edge update rate. We then propose a system identification method for parameter estimation of the bilinear ODEs of our model, and we test the model performance on a Japanese COVID-19 dataset by generating the trajectories of the age-wise numbers of infected individuals in the prefecture of Tokyo for a period of over 365 days. In the process, we also develop an algorithm to identify the different \textit{phases} of the pandemic, each phase being associated with a unique set of contact rates. Our results show a good agreement between the generated trajectories and the observed ones.

==> p_star.tex <==
\section{Revisiting Class $\mathcal P^*$: A Special Class of Stochastic Chains}\label{sec:p_star}
We are at the point of deviating from the standard strong connectivity assumptions for social learning~\cite{jadbabaie2012non,liu2014social,liu2012social,zhao2012learning}. In order to understand the challenges involved in this process, first note that \eqref{eq:main} can also be expressed as follows (see equation (4) in~\cite{jadbabaie2012non}):
\begin{align}\label{eq:vector_form}
    &\mu_{t+1}(\theta) - A(t)\mu_t(\theta)=\text{diag}\left(\ldots,a_{ii}(t)\left[\frac{l_i(\omega_{i,t+1}|\theta)}{m_{i,t}(\omega_{i,t+1})}-1\right],\ldots\right)\mu_t(\theta),
\end{align}
\blue{where $m_{i,t}(s):=m_{i,t}^{(1)}(s)$ for all $s\in S_i$.} Now, suppose $\theta=\theta^*$. Then, by extrapolation of the known results for non-Bayesian learning, we expect that the right-hand-side of~\eqref{eq:vector_form} decays to 0 almost surely as $t\rightarrow\infty$. This means that for large values of $t$ (say $t\geq T_0$ for some $T_0\in\N$), the dynamics~\eqref{eq:vector_form} for $\theta=\theta^*$ can be approximated as: $\mu_{t+1}(\theta^*)\approx A(t)\mu_t(\theta^*)$. Hence, we expect the limiting value of $\mu_t(\theta^*)$ to be closely related to $\lim_{t\rightarrow\infty}A(t:T_0)$, whenever the latter limit exists. However, without the standard assumptions on network connectivity, it is often challenging to gauge the existence of limits of backward matrix products such as $A(t:T_0)$. 

To overcome this difficulty, we use the notion of Class $\pstar$ introduced in~\cite{touri2012product}. This notion is based on Kolmogorov's ingenious concept of absolute probability sequences, which we now define. 
% \begin{definition}  [\textbf{Absolute Probability Sequence}] \label{def:abs_prob_seq} A sequence of stochastic vectors $\{\pi(t)\}_{t=0}^\infty$ is said to be an absolute probability sequence for a deterministic stochastic chain $\{A(t)\}_{t=0}^\infty$ if
% $$
% \pi^T(t+1)A(t) = \pi^T(t)\quad\text{for all }t\in\N_0.
% $$
% % \end{definition}
% Conceptually, absolute probability processes are extensions of absolute probability sequences to random stochastic chains. To make this precise, let $\F\subset 2^{\Omega_2}$ be a $\sigma$-field and let $P$ be a probability measure such that $(\Omega_2,\F,P)$ is a probability space. Let $\{A(t)\}_{t=0}^\infty$ be a random stochastic chain that is measurable w.r.t. $\F$. For each $t\in\mathbb N$, let $\F_t:=\sigma(A(0),A(1),\ldots, A(t-1))$. Further, let $\E$ be the expectation operator w.r.t. $P$. We then have the following.

\begin{definition}  [\textbf{Absolute Probability Sequence} \cite{touri2012product}] \label{def:abs_prob_seq} Let $\{A(t)\}_{t=0}^\infty$ be either a deterministic stochastic chain or a random process of independently distributed stochastic matrices.
A deterministic sequence of stochastic vectors $\{\pi(t)\}_{t=0}^\infty$ is said to be an absolute probability sequence for $\{A(t)\}_{t=0}^\infty$ if 
$$
\pi^T(t+1)\E[A(t)]=\pi^T(t)\quad\text{for all } t\geq 0.
$$
\end{definition}
Note that every deterministic stochastic chain admits an absolute probability sequence \cite{kolmogoroff1936theorie}. Hence, every random sequence of independently distributed stochastic matrices also admits an absolute probability sequence. 

Of interest to us is a special class of random stochastic chains which are associated with absolute probability sequences satisfying a certain condition. This class of chains is called Class $\pstar$, as defined below. 

\begin{definition} [\textbf{Class $\mathbf{\mathcal{P}^*}$} \label{def:pstar} \cite{touri2012product}] We let (Class-)$\mathcal P^*$ be the set of random stochastic chains with an absolute probability sequence $\{\pi(t)\}_{t=0}^\infty$ such that $\pi(t)\geq p^*\mathbf 1$ for some scalar $p^*>0$ and all $t\in\N_0$. (Note that the absolute probability sequence and the value of $p^*$ may vary from chain to chain). 
\end{definition}
% Note that a deterministic stochastic chain $\{A(t)\}_{t=0}^\infty$ belongs to Class $\pstar$ iff there exist for $\{A(t)\}_{t=0}^\infty$ an absolute probability \textit{sequence} $\{\pi(t)\}_{t=0}^\infty$ and a scalar $p^*>0$ such that $\pi(t)\geq p^*\allone$ for all $t\in\N_0$.

\blue{It is worth noting that in the context of social learning, if $\{\pi(t)\}_{t=0}^\infty$ is an absolute probability sequence for $\{A(t)\}_{t=0}^\infty$, then $\pi_i(t)$ denotes the \textit{Kolmogorov centrality} or \textit{social power} of agent $i$ at time $t$, which quantifies how influential the $i$-th agent is relative to other agents at time $t$~\cite{touri2012product,molavi2017foundations}. In view of Definition~\ref{def:pstar}, this means that, if a stochastic chain belongs to Class $\pstar$, then the expected chain describes a sequence of influence graphs in which the social power of every agent exceeds a fixed positive threshold $p^*$ at all times.}
\blue{We now look at some concrete examples of Class $\pstar$ chains.}
\blue{\begin{example}\label{eg:doubly_stochastic}
 Let $\mathcal D\subset\R^{n\times n}$ be a finite collection of doubly stochastic matrices. Let $\{A(t)\}_{t=0}^\infty$ be a sequence of i.i.d. random matrices, each of which is uniformly distributed on $\mathcal D$. Then $\{A(t)\}_{t=0}^\infty$ belongs to Class $\pstar$, as shown below.\\
 \indent Observe that $\frac{1}{n}\allone^T A(t) = \frac{1}{n}\allone^T$ due to double stochasticity. Hence, $\left(\frac{1}{n}\allone, \frac{1}{n}\allone,\ldots\right )$ is an absolute probability sequence for $\{A(t)\}_{t=0}^\infty$. Setting $p^*=\frac{1}{n}$ now shows that $\{A(t)\}_{t=0}^\infty\in\pstar$.
\end{example}
\begin{example}\label{eg:not_balanced}
Suppose $A(t)=A_e$ for all even $t\in\N_0$, and $A(t) = A_o$ for all odd $t\in \N_0$, where $A_e$ and $A_o$ are the matrices defined below:
\[ A_e := \left( \begin{array}{cc}
1 & 0 \\
\frac{1}{2} & \frac{1}{2}
\end{array} \right), \quad A_o:=
%
\left( \begin{array}{cc}
\frac{1}{2} & \frac{1}{2} \\
0 & 1
\end{array} \right).
\]
Then one may verify that the alternating sequence $[\frac{2}{3}\,\,\frac{1}{3}]^T,[\frac{1}{3}\,\,\frac{2}{3}]^T, [\frac{2}{3}\,\,\frac{1}{3}]^T,\ldots$ is an absolute probability sequence for the chain $\{A(t)\}_{t=0}^\infty$. Hence, $\{A(t)\}_{t=0}^\infty\in \pstar$.\\
\indent Let us now add a zero-mean independent noise sequence $\{W(t)\}_{t=0}^\infty$ to the original chain, where for all even $t\in\N_0$, the matrix $W(t)$ is the all-zeros matrix (and hence a degenerate random matrix), and for all odd $t\in\N_0$, the matrix $W(t)$ is uniformly distributed on $\{W_0, -W_0\}$, with $W_0$ given by
$$ W_0 := 
\begin{pmatrix}
-\frac{1}{2} & \frac{1}{2}\\
0 & 0
\end{pmatrix}.
$$
Then by Theorem 5.1 in~\cite{touri2012product}, the random stochastic chain $\{A(t) + W(t) \}_{t=0}^\infty$ belongs to Class $\pstar$ because the expected chain $\{\E[A(t) + W(t)] \}_{t=0}^\infty= \{A(t)\}_{t=0}^\infty$ belongs to Class $ \pstar$.
\end{example}
\begin{remark}\label{rem:random_not_deterministic} Interestingly, Example~\ref{eg:not_balanced} illustrates that a random stochastic chain may belong to Class $\pstar$ even though almost every realization of the chain lies outside Class $\pstar$. To elaborate, consider the setup of Example~\ref{eg:not_balanced}, and let $\tilde A(t):=A(t) + W(t)$. Observe that $A_o - W_0=I$, which means that for any $B\in \N$ and $t_1\in \N_0$, the probability that $A(t) + W(t) = I$ for all odd $t\in \{t_1,\ldots, t_1+2B-1\}$ is  $\left(\frac{1}{2} \right)^B>0$. Since $\{W(t)\}_{t=0}^\infty$ are independent, it follows that for $\mathbb P^*$-almost every realization $\{\hat A(t)\}_{t=0}^\infty$ of $\{\tilde A(t)\}_{t=0}^\infty$, there exists a time $\tau\in \N_0$ such that $\hat A(\tau + 2B:\tau) = A_e\cdot I\cdot A_e\cdot I\cdots A_e\cdot I = A_e^B$. Therefore, if $\{\pi_R(t)\}_{t=0}^\infty$ is an absolute probability sequence for the deterministic chain $\{\hat A(t)\}_{t=0}^\infty$, we can use induction along with Definition~\ref{def:abs_prob_seq} to show that $\pi_R^T(\tau) = \pi_R^T(\tau+2B)\hat A(\tau+2B:\tau)$. Thus,
$$
\pi_R^T(\tau) = \pi_R^T(\tau+2B) A_e^B \leq \allone^T  A_e^B.
$$
Since the second entry of $\allone^T A_e^B$ evaluates to $\frac{1}{2^B}$, and since $B$ is arbitrary, it follows that there is no lower bound $p^*>0$ on the second entry of $\pi_R(\tau)$. Hence, $\{\hat A(t)\}_{t=0}^\infty\notin\pstar$, implying that $\mathbb P^*$-almost no realization of $\{\tilde A(t)\}$ belongs to Class $\pstar$.
\end{remark}}

\blue{We now turn to a noteworthy subclass of Class $\pstar$: the class of \textit{uniformly strongly connected} chains (Lemma 5.8,~\cite{touri2012product}). } Below is the definition of this subclass (reproduced from~\cite{touri2012product}).

\begin{definition}[\textbf{Uniform Strong Connectivity}]\label{def:unif_strong_connect}  A deterministic stochastic chain $\{A(t)\}_{t=0}^\infty$ is said to be uniformly strongly connected if:
\begin{enumerate}
    \item there exists a $\delta>0$ such that for all $i,j\in[n]$ and all $t\in\N_0$, either $a_{ij}(t)\geq \delta$ or $a_{ij}(t)=0$,
    \item \label{item:strong_feedback} $a_{ii}(t)>0$ for all $i\in[n]$ and all $t\in \N_0$, and
    \item \label{item:b_strong} there exists a constant $B\in\N$ such that the sequence of directed graphs $\{G(t)\}_{t=0}^\infty$, defined by $G(t) = ([n], E(t))$ where $ E(t):=\{ (i,j)\in [n]^2: a_{ji}(t)>0\}$, has the property that the graph:
    $$
        \G(k):=\left([n], \bigcup_{q=kB}^{(k+1)B-1} E(q)\right )
    $$
    is strongly connected for every $k\in \N_0$.
\end{enumerate}
\end{definition}
Due to the last requirement above, uniformly strongly connected chains are also called $B$-strongly connected chains or simply $B$-connected chains. Essentially, a uniformly strongly connected chain describes a time-varying network that may not be connected at every time instant but is guaranteed to be connected over bounded time intervals that occur periodically.

Besides uniformly strongly connected chains, we are also interested in another subclass of Class $\pstar$: the set of independent \textit{balanced} chains with \textit{feedback property} (Theorem 4.7, ~\cite{touri2012product}). The italicised terms are defined below.

\begin{definition}[\textbf{Balanced chains}] \label{def:balanced_chains} A stochastic chain $\{A(t)\}_{t=0}^\infty$ is said to be balanced if there exists an $\alpha>0$ such that:
\begin{equation}\label{eq:balance}
    \sum_{i\in C}\sum_{j\in [n]\setminus C} a_{ij}(t) \geq \alpha \sum_{i\in [n]\setminus C}\sum_{j\in C} a_{ij}(t)
\end{equation}
for all sets $C\subset[n]$ and all $t\in\N_0$.
\end{definition}

\begin{definition} [\textbf{Feedback property}] We say that a random stochastic chain, $\{A(t)\}_{t=0}^\infty$ has feedback property if there exists a $\delta>0$ such that
$$
    \E[a_{ii}(t) a_{ij}(t)|\F_t]\geq \delta \E[a_{ij}(t)|\F_t]\quad\textit{a.s.}
$$
for all $t\in\N_0$ and all distinct $i,j\in[n]$.
\end{definition}

Intuitively, a balanced chain is a stochastic chain in which the total influence of any subset of agents $C\subset[n]$ on the complement set $\bar C:=[n]\setminus C$ is neither negligible nor tremendous when compared to the total influence of $\bar C$ on $C$. Since the definition of feedback property is rather abstract, we relate it to the \textit{strong feedback property}, which has a clearer interpretation. This term is defined below.
\begin{definition} [\textbf{Strong feedback property}]
We say that a random stochastic chain $\{A(t)\}_{t=0}^\infty$ has the strong feedback property with feedback coefficient $\delta$ if there exists a $\delta>0$ such that $a_{ii}(t)\geq \delta$ \textit{a.s.} for all $i\in [n]$ and all $t\in\N_0$.
\end{definition}
Intuitively, a chain with the strong feedback property describes a network in which all the agents' self-confidences are always above a certain threshold.

To see how the strong feedback property is related to the (regular) feedback property, note that by Lemma 4.2 of~\cite{touri2012product}, if $\{A(t)\}_{t=0}^\infty$ has feedback property, then the expected chain, $\{\E[A(t)]\}_{t=0}^\infty$ has the strong feedback property. Thus, a balanced independent chain with feedback property describes a network in which complementary sets of agents influence each other to comparable extents, and every agent's mean self-confidence is always above a certain threshold.
\blue{
\begin{remark} \label{rem:first}
It may appear that every stochastic chain belonging to Class $\pstar$ is either uniformly strongly connected or  balanced with feedback property, but this is not true. Indeed, one such chain is described in Example~\ref{eg:not_balanced}, wherein we have $A(t)+W(t)=A_e$ for even $t\in\N_0$, which implies that~\eqref{eq:balance} is violated at even times. Hence, $\{A(t)+W(t)\}_{t=0}^\infty$ is not a balanced chain. As for uniform strong connectivity, recall from Remark~\ref{rem:random_not_deterministic} that $\mathbb P^*$-almost every realization of $\{A(t)+W(t)\}_{t=0}^\infty$ lies outside Class $\pstar$. Since Class $\pstar$ is a superset of the class of uniformly strongly connected chains, it follows that $\{A(t)+W(t)\}_{t=0}^\infty$ is almost surely not uniformly strongly connected.
\end{remark}
\begin{remark}\label{rem:second}
Another example of Class $\mathcal P^*$ chains that are not uniformly strongly connected comes from Example~\ref{eg:doubly_stochastic}. To see how, recall the notation of Example~\ref{eg:doubly_stochastic} and suppose that $I\in \mathcal D$. %(which is possible because the identity matrix is doubly stochastic). 
Then, for any $B\in \N$ and $t_1\in \N_0$, the probability that $A(t)=I$ for all $t\in\{t_1,\ldots, t_1+B-1\}$ equals $\frac{1}{|\mathcal D|^B}$. In light of the independence of $\{A(t)\}_{t=0}^\infty$, this implies that there almost surely exists a time interval of length $B$ during which no agent interacts with others. As $B$ is arbitrary, this means that the chain $\{A(t)\}_{t=0}^\infty$ is almost surely not uniformly strongly connected. 
\end{remark}}
